Existence and Completeness of Solutions to Extended Projected Dynamical Systems and Sector-bounded Projection-based Controllers

Projection-based control (PBC) systems have significant engineering impact and receive considerable scientific attention. To properly describe closed-loop PBC systems, extensions of classical projected dynamical systems are needed, because partial projection operators and irregular constraint sets (sectors) are crucial in PBC. These two features obstruct the application of existing results on existence and completeness of solutions. To establish a rigorous foundation for the analysis and design of PBC, we provide essential existence and completeness properties for this new class of discontinuous systems.

==> commands.tex <==

\newcommand{\Rl}[2]{\ensuremath{\mathbb{R}^{#1}_{#2}}}   % Euclidean space
\newcommand{\Rlp}{\ensuremath{\mathbb{R}_{>0}}}
\newcommand{\Rlo}{\ensuremath{\mathbb{R}_{\geq 0}}}
\newcommand{\Zo}{\ensuremath{\mathbb{N}_{0}}}
\newcommand{\Zp}{\ensuremath{\mathbb{N}_{> 0}}}
\newcommand{\C}[1]{\ensuremath{\mathbb{C}^{#1}}}         % Complex plane
\newcommand{\N}{\ensuremath{\mathbb{N}}}                 % Set of natural numbers
%\newcommand{\No}{\ensuremath{\mathbb{N}_{0}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}


%\definecolor{bleucit}{rgb}{0.2,0.4,0.6} % nouvelle couleur
%\newcommand\sblue[1]{{\color{bleucit}#1}} %sblue stands for `sweet blue'
%\newcommand{\bleucit}{\textcolor{bleucit}}
\newcommand\cp[1]{{`\emph{#1}'}}
\newcommand\blue[1]{\emph{{\color{blue}#1}}}


\newcommand{\dst}{\displaystyle}
\newcommand{\Linf}[1]{\ensuremath{\mathcal{L}^{#1}}}

\newcommand{\eg}{{\it e.g.}}

\newcommand{\KL}{\ensuremath{\mathcal{KL}}}
\newcommand{\K}{\ensuremath{\mathcal{K}}}
\newcommand{\Kinf}{\ensuremath{\mathcal{K}_{\infty}}}
\newcommand{\KK}{\ensuremath{\mathcal{KK}}}
\newcommand{\KKL}{\ensuremath{\mathcal{KKL}}}
\newcommand{\KLL}{\ensuremath{\mathcal{KLL}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}
\newcommand{\PD}{\ensuremath{\mathcal{PD}}}

% Flow and jump sets
\newcommand{\Cs}{\ensuremath{C_{\text{steady}}}}
\newcommand{\Ct}{\ensuremath{C_{\text{transient}}}}
\newcommand{\Ds}{\ensuremath{D_{\text{steady}}}}
\newcommand{\Dt}{\ensuremath{D_{\text{transient}}}}
\newcommand{\UtGpAS}{U$_{\text{t}}$GpAS}
\newcommand{\UtGAS}{U$_{\text{t}}$GAS}
\newcommand{\UjGpAS}{U$_{\text{j}}$GpAS}
\newcommand{\UjGAS}{U$_{\text{j}}$GAS}

\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\argmin}{argmin}
%\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\pos}{pos}
\providecommand{\mh[1]}{{\color{blue}#1}}

%\newcommand{\d}{\ensuremath{\delta}}

\newcommand{\interior}{\ensuremath{\text{int}\,}}
\newcommand{\dom}{\ensuremath{\text{dom}\,}}
\newcommand{\co}{\ensuremath{\text{co}\,}}
\newcommand{\coc}{\ensuremath{\overline{\text{dom}}\,}}
\newcommand{\ext}{\ensuremath{\text{ext}}}
\newcommand{\rge}{\ensuremath{\text{rge}\,}}
\newcommand{\esup}{\ensuremath{\text{ess.sup}\,}}


\newcommand{\sign}[1]{\ensuremath{\text{sign}{(#1)}}}
\newcommand{\sat}{\ensuremath{\text{sat}}}

\newcommand{\sinc}{\ensuremath{\text{sinc}}}
\newcommand{\nom}{\ensuremath{\text{nom}}}


\newcommand{\Tmati}{\ensuremath{T_{MATI}\,\,}}
\newcommand{\Tmasp}{\ensuremath{\mathrm{T_{MASP}}\,}}
\newcommand{\lc}{\ensuremath{\llbracket}}
\newcommand{\rc}{\ensuremath{\rrbracket}}
%\newcommand{\arg}{\ensuremath{\text{arg}}}
%

\newcommand{\norm}[1]{\ensuremath{\left\|{#1}\right\|}}
\newcommand{\ip}[2]{\ensuremath{\left\langle #1, #2\right\rangle}}
\newcommand{\cb}[1]{\ensuremath{\overline{\mathbb{B}}_{\mbox{\scriptsize $#1$}}}}                              % Closed unit ball
\newcommand{\ob}[2]{\ensuremath{\mathbb{B}_{\mbox{\scriptsize $#1$}}\ensuremath{\left( #2\right)}}}   % Open unit ball
\newcommand{\df}{\ensuremath{\stackrel{\mbox{\tiny $\mathrm{def}$}}{=}\:}}                                             % Defined by
\newcommand{\myint}[4]{\ensuremath{\int_{#1}^{#2}#3\;\mathrm{d}#4}}
\newcommand{\Mm}{\ensuremath{\:\stackrel{\rightarrow}{\scriptstyle{\rightarrow}}\:}}
\newcommand{\bm}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\hs}[1]{\hspace*{#1 em}}
%\newcommand{\summ}{\ensuremath{\sum_{i\in\mathcal{I}}}}
\newcommand{\qa}{\ensuremath{\mathcal{Q}_{A}}}%
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\di}{\ensuremath{\mathcal{D}_{i}}}


%
%\newcounter{eq}
%\newcommand{\arabalph}{\stepcounter{equation}%
%\setcounter{eq}{\value{equation}}%
%\setcounter{equation}{0}%
%\renewcommand{\theequation}{\theeq\alph{equation}}}
%\newcommand{\arab}{\setcounter{equation}{\value{eq}}%
%\renewcommand{\theequation}{\arabic{equation}}}

%\newtheoremstyle{note}% name
%  {3pt}%      Space above
%  {3pt}%      Space below
%  {}%         Body font
%  {}%         Indent amount (empty = no indent, \parindent = para indent)
%  {\itshape}% Thm head font
%  {:}%        Punctuation after thm head
%  {.5em}%     Space after thm head: " " = normal interword space;
%        %       \newline = linebreak
%  {}%         Thm head spec (can be left empty, meaning `normal')
%
%\theoremstyle{note}
%\newtheorem{note}{Note}


% Commandes d'Adolfo
\newcommand{\ie}{{\it i.e.}}
%\newcommand{\eg}{{\it e.g. }}


%\newcommand{\ree}{\mathbb{R}}
\newcommand{\nat}{\mathbb{N}}

%
%\usepackage{amsthm}
%\newtheorem{defn}{Definition}
%\newtheorem{claim}{Claim}
%\newtheorem{hypo}{Hypothesis}
%\newtheorem{ass}{Assumption}
%\newtheorem{prop}{Proposition}
%\newtheorem{fact}{Fact}
%\newtheorem{lem}{Lemma}
%
%\newtheorem{thm}{Theorem}
%\newtheorem{cor}{Corollary}
%\newtheorem{pb}{Problem}
%%\newtheorem{proof}{Proof}[section]
%
%\theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\newenvironment{rem}{\begin{remark}}{\hfill $\Box$\end{remark}}
%\newtheorem{exam}{Example}
%\newenvironment{ex}{\begin{exam}}{\hfill $\Box$\end{exam}}
%\newenvironment{pf}[1]{\begin{IEEEproof}#1}{\end{IEEEproof}}
%\renewcommand{\IEEEproofindentspace}{0\parindent}
%\renewcommand\IEEEproofname{\textbf{Proof}}

%\newtheorem{exple}{Example}[section]
%\newtheorem{defn}{Definition}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{hypo}{Hypothesis}[section]
%\newtheorem{ass}{Assumption}[section]
%\newtheorem{prop}{Proposition}[section]
%\newtheorem{fact}{Fact}[section]
%\newtheorem{lem}{Lemma}[section]
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{cor}{Corollary}[section]
%%\newtheorem{proof}{Proof}[section]
%\newtheorem{rem}{Remark}[section]



%
%  Remark environment
%
%\newenvironment{rem}{\textit{Remark. }}{\mbox{}\\[1ex]}
\newenvironment{rems}{\textit{Remarks. }}{\mbox{}\\[1ex]}
%

